Identity and Granularity of Events in Text

In this paper we describe a method to detect event descrip- tions in different news articles and to model the semantics of events and their components using RDF representations. We compare these descriptions to solve a cross-document event coreference task. Our com- ponent approach to event semantics defines identity and granularity of events at different levels. It performs close to state-of-the-art approaches on the cross-document event coreference task, while outperforming other works when assuming similar quality of event detection. We demonstrate how granularity and identity are interconnected and we discuss how se- mantic anomaly could be used to define differences between coreference, subevent and topical relations.

==> model.tex <==
\section{A model for event identity and granularity}
\label{sec:model}

We model events as a combination of five slots, as annotated in the ECB+ data set (\cite{CYBULSKA+VOSSEN:2014}) used in the experiments. The five slots correspond to different elements of event information such as the action slot (or event trigger following the ACE (\cite{ACE-event-2005}) terminology) and four kinds of event arguments: time, location, human and non-human participant slots (see \cite{CYBULSKA2014nwr1}).

The approach described here determines coreference between mentions of events through compatibility of slots of the five slot template. The next quote shows an excerpt from topic one, text number seven of the ECB corpus (\cite{Bejan-Harabagiu-2010}).
\begin{quotation}
\textit{The ``American Pie" actress has entered Promises for undisclosed reasons. The actress, 33, reportedly headed to a Malibu treatment facility on Tuesday.}
\end{quotation}
Consider two event templates presenting the distribution of event information over the five event slots in the two example sentences (tables \ref{tab:ecb-1} and \ref{tab:ecb-2}).

\begin{table}[htp]
\caption{Sentence template ECB topic 1, text 7, sentence 1}
{\scriptsize 
\begin{center}
\begin{tabular}{|l|l|}
\hline
Action & \textit{entered}\\
Time &  N/A\\
Location &  \textit{Promises}\\
Human Participant & \textit{actress}\\
Non-Human Participant & N/A\\
\hline
\end{tabular}
\end{center}
}
\label{tab:ecb-1}
\end{table}%

\begin{table}[htp]
\caption{Sentence template ECB topic 1, text 7, sentence 2}
{\scriptsize 
\begin{center}
\begin{tabular}{|l|l|}
\hline
Action & \textit{headed}\\
Time & \textit{on Tuesday}\\
Location & \textit{to a Malibu treatment facility}\\
Human Participant & \textit{actress}\\
Non-Human Participant&  N/A\\
\hline
\end{tabular}
\end{center}
}
\label{tab:ecb-2}
\end{table}%

If event mentions are coreferent, they refer to the same event instance. Two or more event mentions are coreferent if they describe actions that happen or hold true in the same time and place and with involvement of the same participants.

Coreferent event mentions share the same granularity. (XXX: America - American President? REMOVE THE LAST SENTENCE OR EXTEND THIS.)



